Neural Language Modeling for Contextualized Temporal Graph Generation

This paper presents the first study on using large-scale pre-trained language models for automated generation of an event-level temporal graph for a document. Despite the huge success of neural pre-training methods in NLP tasks, its potential for temporal reasoning over event graphs has not been sufficiently explored. Part of the reason is the difficulty in obtaining large training corpora with human-annotated events and temporal links. We address this challenge by using existing IE/NLP tools to automatically generate a large quantity (89,000) of system-produced document-graph pairs, and propose a novel formulation of the contextualized graph generation problem as a sequence-to-sequence mapping task. These strategies enable us to leverage and fine-tune pre-trained language models on the system-induced training data for the graph generation task. Our experiments show that our approach is highly effective in generating structurally and semantically valid graphs. Further, evaluation on a challenging hand-labeled, out-domain corpus shows that our method outperforms the closest existing method by a large margin on several metrics. Code and pre-trained models are available at https://github.com/madaan/temporal-graph-gen.

==> notes.tex <==
1. Use existing IR techniques to create dataset

2. CAEVO's generated data has inductive bias, unavoidably lots of errors and noise. 

3. We augment human knowledge to the labels to reduce the noise and improve the quality of the label data.
- improve signal to noise ratio

4. We feed this data to strong learners, showcasing that strong models are able to learn

5. Graphs generated by those systems are not fit for downstream consumption.

6. Add human prunings and clustering for cleaning up the data: collecting less trivial events.

7. The cleaning allows you to reduce X\% of the noisy events

8. Evaluate to test how much are you able to get.


9. We create a dataset that is effective.

10. We can generalize from these examples to learn something, they still
low cost of development, low cost of data, relative performance of system's ability when you learn from imperfect data]


While this is an important task, it has not gained much attention. Major bottlenecks for transferring the advances in large pre-trained language model is that there is not enough data. We break this barrier by outlining a pipeline to generate affordable semi-supervised data for the task. 
We then outline a set of pruning and augmentation procedures that improve the signal/noise ratio of the data and make it more well defined.
We hope that these operations help in reducing the inductive bias of \caevo.
We then represent each graph as a string using \dot, and use masked-languae modeling with \gptz. We show large gains, showing that our data has effective signals.

Related work:

- Clearly differentiate COMET, Jurafsky merge with graph generation and differentiate. 


==> tasks.tex <==
\section{Background and Task Description}


==> todo.tex <==
\section{To-do}
\begin{itemize}
    \item Only focus on salient events. Consider domain as well as granularity.
    \item Generative metrics.
    \item Generate nodes first. In general, explore which order of factorization works the best? Are there advantages to using certain orderings?
    \item CAVEO is a straight forward baseline
    \item Using summary to find salient events.
    \item Graph induction where the nodes scores are given by a summarizing framework, and edge weights are given by CAEVO.
    \item Tree-based decoding
    \item Graph-data generation.
    \item Perform document-level generation by using the following inductive-bias: most sub-graphs would only depend on 2-3 sentences. Generate these subgraphs, and then have a module that can predict links between these smaller subgraphs (or have a further inductive bias).
    \item One neural baseline: predict events and then predict edges.
\end{itemize}
